Exploring Graph Structure Comprehension Ability of Multimodal Large Language Models: Case Studies

Large Language Models (LLMs) have shown remarkable capabilities in processing various data structures, including graphs. While previous research has focused on developing textual encoding methods for graph representation, the emergence of multimodal LLMs presents a new frontier for graph comprehension. These advanced models, capable of processing both text and images, offer potential improvements in graph understanding by incorporating visual representations alongside traditional textual data. This study investigates the impact of graph visualisations on LLM performance across a range of benchmark tasks at node, edge, and graph levels. Our experiments compare the effectiveness of multimodal approaches against purely textual graph representations. The results provide valuable insights into both the potential and limitations of leveraging visual graph modalities to enhance LLMs' graph structure comprehension abilities.

==> pages/related_work.tex <==
\textbf{Graph Structure Comprehension with Text Modality LLMs.}
Recent advancements in LLMs have increased interest in their application to graph-structured data~\cite{XWLZW24, ZZM242}. 
A representative work by \citet{FHP24} introduces GraphQA, a comprehensive benchmark for evaluating LLMs' ability to reason about graph structures when presented with textual graph descriptions. 
Their study explored various text-based graph encoding methods and prompt engineering techniques, demonstrating that carefully designed textual representations can enable LLMs to perform a range of graph reasoning tasks. 
These studies collectively highlight the growing capability of text-based LLMs in understanding and reasoning about graph structures while also revealing limitations in their ability to fully capture the inherent visual and relational nature of graphs.

\textbf{Graph Structure Comprehension with Multimodal LLMs.}
The emergence of multimodal Large Language Models, capable of processing both text and visual information, has opened new avenues for graph structure comprehension. However, research specifically focusing on using multimodal LLMs for graph understanding is still in its nascent stages~\cite{WFJKZ24, WC24, CMLJ23}. 
Some related work in this area includes the study by \citet{DGSK23}, which explored the influence of graph multimodalities on LLM performance, although their focus was not specifically on graph structure comprehension. 
% 
Our work aims to address these gaps by extending existing text-based benchmarks to include visual graph representations, thereby providing a foundation for future research in this emerging field.

